DeepJoin: Joinable Table Discovery with Pre-trained Language Models

Due to the usefulness in data enrichment for data analysis tasks, joinable table discovery has become an important operation in data lake management. Existing approaches target equi-joins, the most common way of combining tables for creating a unified view, or semantic joins, which tolerate misspellings and different formats to deliver more join results. They are either exact solutions whose running time is linear in the sizes of query column and target table repository or approximate solutions lacking precision. In this paper, we propose Deepjoin, a deep learning model for accurate and efficient joinable table discovery. Our solution is an embedding-based retrieval, which employs a pre-trained language model (PLM) and is designed as one framework serving both equi- and semantic joins. We propose a set of contextualization options to transform column contents to a text sequence. The PLM reads the sequence and is fine-tuned to embed columns to vectors such that columns are expected to be joinable if they are close to each other in the vector space. Since the output of the PLM is fixed in length, the subsequent search procedure becomes independent of the column size. With a state-of-the-art approximate nearest neighbor search algorithm, the search time is logarithmic in the repository size. To train the model, we devise the techniques for preparing training data as well as data augmentation. The experiments on real datasets demonstrate that by training on a small subset of a corpus, Deepjoin generalizes to large datasets and its precision consistently outperforms other approximate solutions'. Deepjoin is even more accurate than an exact solution to semantic joins when evaluated with labels from experts. Moreover, when equipped with a GPU, Deepjoin is up to two orders of magnitude faster than existing solutions.

==> response-mr.tex <==
We appreciate the meta-reviewer and the reviewers' comments and
suggestions that help us to improve the quality of the paper. We 
made the following major revisions requested the meta-reviewer.

\begin{itemize}
  \item We revised the technical part of the paper (Sections 
  \ref{sec:model} and \ref{sec:train}). In particular, we added 
  a working example in Section~\ref{sec:model} to illustrate how 
  \deepjoin, the proposed method, works.
  \item We added a baseline method, TURL~\cite{turl}, in the experiments 
  (Section \ref{sec:exp}) and fed the comparison with baselines by 
  showing win/loss examples (Section~\ref{sec:exp:accuracy}) to 
  illustrate the advantage of \deepjoin. 
  \item We provided more thorough analysis and a more detailed 
  explanation of the experiments (Section~\ref{sec:exp:accuracy}). 
\end{itemize}

Major changes in the revised paper are marked in \revise{blue}. 
In addition, since this submission has been moved from Scalable Data 
Science Track to Regular Research Track, with four more pages available, 
the supplementary materials provided with an external link in the first 
submission are also available in this revision. 
Next, we provide our responses to reviewers' comments. 
% except for minor comments (e.g., replotting figures) that have been fixed. 
References to the revised paper are marked in \reviseref{red}. 

==> response-r2.tex <==
\section*{Reviewer \#2}

\review{\heada{W1}%
Substantial extension of the presentation.
}

\headb{Response:}%
To improve the presentation, we added a working example in \reviseref{Section~\ref{sec:model}}. 
This example covers column-to-text transformation, column embedding, and searching. 
Please refer to \reviseref{Examples~\ref{ex:column-to-text} and \ref{ex:index-and-search}}. 

\review{\heada{W2}%
Deeper analysis of the experiments.
}

\headb{Response:}%
We added more analysis of experimental results by drilling down the types of 
joinable columns. As per the request in the review comments, we consider key-foreign 
key joins for data cleaning (near duplicate) references and key-foreign key joins 
for related columns (attribute enrichment). \deepjoin consistently outperforms other 
methods, and the advantage is remarkable for both types. Please refer to 
\reviseref{Table~\ref{tab:join-case-drill-down}} and the analysis in 
\reviseref{Section~\ref{sec:exp:accuracy}.}

For the case of similar coordinates, the join does not pertain to semantic similarity but 
spatial similarity. Hence, we believe that rather than fine-tuning a PLM, which excels 
handling semantics, a better solution to this case is column type annotation followed by a 
spatial join. Column type annotation can detect coordinate attributes in tables. Notable 
approaches are Sherlock~\cite{sherlock}, Sato~\cite{sato}, and DODUO~\cite{doduo}. For 
spatial joins, one may refer to \cite{spatial-joins} for a survey. In general, we focus on 
textual attributes in this work. For numerical attributes, a typical solution is utilizing 
the statistical feature vector in Sherlock~\cite{sherlock}, which converts a numerical 
column to a vector, and then we can invoke a vector search to look for joinable columns 
having similar statistics to the query column. In this revision, we added a discussion 
for numerical attributes in \reviseref{Section~\ref{sec:problem-definition}}. 

\review{\heada{D1}%
More explanation of Table~\ref{tab:column-to-text}.
}

\headb{Response:}%
We added an explanation of this table with an example (\reviseref{Example~\ref{ex:column-to-text}}).

\review{\heada{D2}%
Recall assessed by the experts \& experiments with varying column sizes.
}

\headb{Response:}%
Due to the large number of columns in the repository (1M for each dataset in 
our experiments), it is too laborious to label every table in the dataset by experts.
Therefore, we follow the method in \cite{recall-search-engine}, 
which is common practice for the evaluation of Web search engines, to 
compute the recall. In particular, we build a retrieved pool by taking the union 
of the tables identified by the compared methods, instead of considering all the 
tables in the repository. Then, we compute recall by
\begin{align*}
    \text{recall} = \frac{\text{\# retrieved joinable columns}}{\text{\# joinable columns in the retrieved pool}}.
\end{align*}
As such, our experts only need to label the tables in the retrieved pool. 


==> response-r3.tex <==
\section*{Reviewer \#3}

\review{\heada{W1}%
Comparison against more related work (TURL~\cite{turl}).
}

\headb{Response:}%
We added \turl as a baseline in the experiments. 
In summary, \turl performs better than \tabert, another table 
representation learning method. However, \turl is consistently 
outperformed by \deepjoin, and remarkable gaps are observed. The 
reason is that \turl is pre-trained for tasks which significantly 
differ from joinable table discovery, and it is pre-trained using 
only entity-focused Wikipedia tables. Please refer to 
\reviseref{Section~\ref{sec:exp}} for the detailed comparison. 

Besides the empirical comparison with \turl, we included more 
related work in \reviseref{Section~\ref{sec:related}}.

\review{\heada{W2}%
Win/lose examples compared to baselines.
}

\headb{Response:}%
In \reviseref{Section~\ref{sec:exp:accuracy}}, we added detailed 
analysis of experimental results by showing three typical win/lose 
examples and analyzing the reasons. 
Please refer to \reviseref{Table~\ref{tab:win-lose-example}} and 
the analysis in \reviseref{Section~\ref{sec:exp:accuracy}}. 

\review{\heada{D1}%
Using cosine similarity for training but Euclidean distance for 
searching. 
}

\headb{Response:}%
We performed an ablation study to try different metric combinations 
for training and searching. Please refer to the results in 
\reviseref{Table~\ref{tab:train-search-metric}} and the report in 
\reviseref{Section~\ref{sec:exp:ablation}}. 


==> response-r4.tex <==
\section*{Reviewer \#4}

\review{\heada{W1, D1}%
Tall columns.
}

\headb{Response:}%
Since PLMs have an input length limit \textsf{max\_seq\_length} 
(e.g., 512 tokens for BERT), in case of a tall input column, we choose 
a frequency-based method, e.g., taking a sample of the most frequent 
cell values from the column, whose number of tokens is just within 
\textsf{max\_seq\_length}. Then, we use the sample for column-to-text 
transformation. The reason is that they are more likely to 
yield join results. Here, the frequency of a cell value is defined as 
document frequency, i.e., the number of target columns in the repository 
that have this cell value. In this paper, we focus on the case when 
columns are modeled as sets. When columns are modeled as multisets, we 
may resort to other frequency-based approaches, such as TF-IDF and 
BM25~\cite{DBLP:books/daglib/0021593}. 

We performed an experiment to evaluate the above frequency-based method of handling tall 
columns. A synthetic dataset is used here because the numbers of tall 
columns in the two real datasets in our experiments, Webtable and 
Wikitable, are small. We compared with two options: random sampling 
a number of cells just within \textsf{max\_seq\_length} tokens and truncating 
to the first \textsf{max\_seq\_length} tokens. The experiment shows that 
the frequency-based method consistently outperforms the other two options.

In this revision, we added a discussion in \reviseref{Section~\ref{sec:embed-column}} 
for handling tall columns and conducted an experiment. Please refer to 
\reviseref{Table~\ref{tab:exp:accuracy-tall-columns}} and 
the last paragraph of \reviseref{Section~\ref{sec:exp:accuracy}} for the 
experimental results. Note that $\size{X}$ in this experiment 
denotes the number of distinct cells in a column, and its range is 512 to 4096. When it is 512, there are more 
than 512 tokens. Thus, all the testcases in this experiment exceed the 
\textsf{max\_seq\_length} limit of our PLMs. 

\review{\heada{D2, Minor errors}%
Column labels of Table~\ref{tab:exp:equi-join} \& grammatical errors.
}

\headb{Response:}%
We fixed them in this revision. 

\review{\heada{D3}%
Performance gain in Table~\ref{tab:exp:time-dataset-size}.
}

\headb{Response:}%
In \deepjoin, columns are transformed to fixed-length vectors so that 
approximate nearest neighbor search (ANNS) 
tools can be used to speed up the 
search process. The main contribution of \deepjoin is that it renders the 
time complexity of the search process independent of query and target column 
lengths~\footnote{Query encoding is still linear in the query column length 
because it takes as input the query column.}. 
In previous works such as \josie~\cite{josie} and \pexeso~\cite{pexeso}, a 
comparison linear in the query and target column lengths is required for each 
candidate identified in the search process. 

As for the software used in this paper, we resort to the pre-trained models at 
Hugging Face~\cite{hugging-face-transformers} (e.g., 
MPNet~\footnote{\url{https://huggingface.co/sentence-transformers/all-mpnet-base-v2}}) 
as our PLMs, and use Sentence-BERT~\cite{sbert}~\footnote{\url{https://www.sbert.net/}} 
library to train column embedding. We use the Faiss library~\cite{faiss} for fast ANNS. 
They have been mentioned in the Environments part of 
\reviseref{Section~\ref{sec:exp:setup}}. We would also like to mention that in 
this paper, we proposed a framework featuring embedding-based retrieval for 
joinable table discovery. Our framework is not limited to the PLMs evaluated in 
the experiments, because the PLM can be regarded as a plug-in in our framework. 
For ANNS, our framework is not limited to the use of the Faiss library either. 
As such, we expect the performance of \deepjoin can be further improved by using 
more advanced PLMs or ANNS algorithms. This point has been mentioned in the 
end of \reviseref{Section~\ref{sec:intro}.}


==> response.tex <==
\twocolumn

\section*{Response to Reviewer Comments}
\vspace{2ex}

\input{response-mr}
\vspace{2ex}
\hrule

\input{response-r2}
\vspace{2ex}
\hrule

\input{response-r3}
\vspace{2ex}
\hrule

\input{response-r4}

\clearpage

==> savespace.tex <==
\usepackage[all=normal, floats, bibnotes, wordspacing, charwidths, indent, lists]{savetrees}

\makeatletter%
%
\skip\footins 8.1pt plus 4pt minus 2pt % Space between last line of text top
                                      % and of first footnote.
\floatsep 5pt plus 2pt minus 2pt        % Space between adjacent floats moved
                                         % to top or bottom of text page.
\textfloatsep 5pt plus 2pt minus 4pt    % Space between main text and floats
                                         % at top or bottom of page.
\intextsep 5pt plus 2pt minus 2pt       % Space between in-text figures and
                                         % text.
%\@maxsep 5pt                            % The maximum of \floatsep,
                                         % \textfloatsep and \intextsep (minus
                                         % the stretch and shrink).
\dblfloatsep 5pt plus 0pt minus 0pt     % Same as \floatsep for double-column
                                         % figures in two-column mode.
\dbltextfloatsep 5pt plus 0pt minus 0pt % \textfloatsep for double-column
                                         % floats.
%\@dblmaxsep 5pt                         % The maximum of \dblfloatsep and
                                         % \dbltexfloatsep.

==> vldbblock.tex <==
%%% do not modify the following VLDB block %%
%%% VLDB block start %%%
\pagestyle{\vldbpagestyle}
\begingroup\small\noindent\raggedright\textbf{PVLDB Reference Format:}\\
\vldbauthors. \vldbtitle. PVLDB, \vldbvolume(\vldbissue): \vldbpages, \vldbyear.\\
\href{https://doi.org/\vldbdoi}{doi:\vldbdoi}
\endgroup
\begingroup
\renewcommand\thefootnote{}\footnote{\noindent
This work is licensed under the Creative Commons BY-NC-ND 4.0 International License. Visit \url{https://creativecommons.org/licenses/by-nc-nd/4.0/} to view a copy of this license. For any use beyond those covered by this license, obtain permission by emailing \href{mailto:info@vldb.org}{info@vldb.org}. Copyright is held by the owner/author(s). Publication rights licensed to the VLDB Endowment. \\
\raggedright Proceedings of the VLDB Endowment, Vol. \vldbvolume, No. \vldbissue\ %
ISSN 2150-8097. \\
\href{https://doi.org/\vldbdoi}{doi:\vldbdoi} \\
}\addtocounter{footnote}{-1}\endgroup
%%% VLDB block end %%%

%%% do not modify the following VLDB block %%
%%% VLDB block start %%%
\ifdefempty{\vldbavailabilityurl}{}{
\vspace{.3cm}
\begingroup\small\noindent\raggedright\textbf{PVLDB Artifact Availability:}\\
The source code, data, and/or other artifacts have been made available at \url{\vldbavailabilityurl}.
\endgroup
}
%%% VLDB block end %%%

==> vldbpaperinfo.tex <==
%% The following content must be adapted for the final version
% paper-specific
\newcommand\vldbdoi{10.14778/3603581.3603587}
\newcommand\vldbpages{2458 - 2470}
% issue-specific
\newcommand\vldbvolume{16}
\newcommand\vldbissue{10}
\newcommand\vldbyear{2023}
% should be fine as it is
\newcommand\vldbauthors{\authors}
\newcommand\vldbtitle{\shorttitle} 
% leave empty if no availability url should be set
\newcommand\vldbavailabilityurl{}
% whether page numbers should be shown or not, use 'plain' for review versions, 'empty' for camera ready
\newcommand\vldbpagestyle{empty} 
